The 2022 n2c2/UW Shared Task on Extracting Social Determinants of Health

Objective: The n2c2/UW SDOH Challenge explores the extraction of social determinant of health (SDOH) information from clinical notes. The objectives include the advancement of natural language processing (NLP) information extraction techniques for SDOH and clinical information more broadly. This paper presents the shared task, data, participating teams, performance results, and considerations for future work. Materials and Methods: The task used the Social History Annotated Corpus (SHAC), which consists of clinical text with detailed event-based annotations for SDOH events such as alcohol, drug, tobacco, employment, and living situation. Each SDOH event is characterized through attributes related to status, extent, and temporality. The task includes three subtasks related to information extraction (Subtask A), generalizability (Subtask B), and learning transfer (Subtask C). In addressing this task, participants utilized a range of techniques, including rules, knowledge bases, n-grams, word embeddings, and pretrained language models (LM). Results: A total of 15 teams participated, and the top teams utilized pretrained deep learning LM. The top team across all subtasks used a sequence-to-sequence approach achieving 0.901 F1 for Subtask A, 0.774 F1 Subtask B, and 0.889 F1 for Subtask C. Conclusions: Similar to many NLP tasks and domains, pretrained LM yielded the best performance, including generalizability and learning transfer. An error analysis indicates extraction performance varies by SDOH, with lower performance achieved for conditions, like substance use and homelessness, that increase health risks (risk factors) and higher performance achieved for conditions, like substance abstinence and living with family, that reduce health risks (protective factors).

==> supplemental_files/cover_letter_resubmit1.tex <==
Kevin Lybarger
Assistant Professor
Department of Information Sciences and Technology
George Mason University
4400 University Dr. MSN 1G8
Fairfax, VA 22030
klybarge@gmu.edu


January 10, 2022


Dr. Suzanne Bakken
Editor-in-Chief
Journal of the American Medical Informatics Association


Dear Dr. Bakken,

I am pleased to resubmit the original research article entitled ``The 2022 n2c2/UW Shared Task on Extracting Social Determinants of Health'' for publication in the Journal of the American Medical Informatics Association Focus Issue on Social Determinants of Health (SDOH) Extraction.

This manuscript summarizes the National NLP Clinical Challenges (n2c2) extraction task, Track 2: Extracting Social Determinants of Health (n2c2/UW SDOH Challenge). We have carefully reviewed the reviewer feedback and updated the manuscript to address as many comments as possible. To address the review feedback, we included additional text and figures. Based on your approval, the manuscript word count is 4,499 (< 4,500 limit from email).

This manuscript has not been previously published and is not under consideration elsewhere. Dr. Özlem Uzuner, Dr Meliha Yetisgen, and I are co-editors on the JAMIA SDOH focus issue. We have no additional conflicts of interest to disclose. Thank you for your consideration.

Sincerely,

Kevin Lybarger
